Beyond English: Evaluating LLMs for Arabic Grammatical Error Correction

Large language models (LLMs) finetuned to follow human instruction have recently exhibited significant capabilities in various English NLP tasks. However, their performance in grammatical error correction (GEC), especially on languages other than English, remains significantly unexplored. In this work, we evaluate the abilities of instruction finetuned LLMs in Arabic GEC, a complex task due to Arabic's rich morphology. Our findings suggest that various prompting methods, coupled with (in-context) few-shot learning, demonstrate considerable effectiveness, with GPT-4 achieving up to $65.49$ F$_{1}$ score under expert prompting (approximately $5$ points higher than our established baseline). Despite these positive results, we find that instruction finetuned models, regardless of their size, are still outperformed by fully finetuned ones, even if they are significantly smaller in size. This disparity highlights substantial room for improvements for LLMs. Inspired by methods used in low-resource machine translation, we also develop a method exploiting synthetic data that significantly outperforms previous models on two standard Arabic benchmarks. Our best model achieves a new SOTA on Arabic GEC, with $73.29$ and $73.26$ F$_{1}$ on the 2014 and 2015 QALB datasets, respectively, compared to peer-reviewed published baselines.

==> Tables/2015_GEC.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrr}\toprule
\multirow{2}{*}{\textbf{Settings}} &\multirow{2}{*}{\textbf{Models}} &\multicolumn{4}{c}{\textbf{Exact Match}} &\multicolumn{4}{c}{\textbf{No Alif / Ya Errors}} &\multicolumn{4}{c}{\textbf{No Punctuation}} &\multicolumn{4}{c}{\textbf{No Puncation and Alif / Ya Errors}} \\\cmidrule{3-18}
& &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} \\\midrule
\multirow{4}{*}{\textbf{Encoder-Only }} &ARBERTv2 &73.10 &55.40 &63.03 &68.71 &56.20 &40.60 &47.14 &52.19 &65.60 &63.00 &64.27 &65.06 &70.52 &40.43 &51.39 &61.38 \\
&ARBERTv2 3 Stage &74.20 &53.80 &62.37 &68.97 &57.30 &38.50 &46.06 &52.20 &66.70 &61.50 &63.99 &65.59 &71.24 &38.50 &49.99 &60.88 \\
&MARBERTv2 &72.90 &54.90 &62.63 &68.41 &56.10 &39.70 &46.50 &51.82 &65.50 &62.70 &64.07 &64.92 &70.81 &39.20 &50.46 &60.98 \\
&MARBERTv2 3 Stage &74.00 &52.70 &61.56 &68.47 &57.20 &37.80 &45.52 &51.88 &66.60 &61.20 &63.79 &65.45 &71.50 &37.70 &49.37 &60.63 \\\cmidrule{2-18}
\multirow{5}{*}{\textbf{Decoder-Only}} &LLama 7B Original &59.59 &38.72 &46.94 &53.79 &34.40 &20.55 &25.73 &30.31 &72.46 &56.88 &63.73 &68.70 &69.01 &35.77 &47.12 &58.19 \\
&Alpaca 7B &50.24 &32.42 &39.41 &45.26 &32.30 &19.23 &24.11 &28.43 &70.34 &66.67 &68.46 &69.57 &66.88 &32.50 &43.74 &55.20 \\
&Vicuna 13B &62.53 &40.90 &49.45 &56.55 &35.55 &21.50 &26.79 &31.44 &75.46 &69.56 &72.39 &74.20 &67.33 &35.33 &46.34 &57.00 \\
&bactrian-x-bloom-7b1-lora &65.46 &42.53 &51.56 &59.09 &52.35 &39.40 &44.96 &49.12 &80.01 &70.45 &74.93 &77.90 &69.55 &36.88 &48.20 &59.08 \\
&bactrian-x-llama-7b-lora &58.35 &40.24 &47.63 &53.53 &48.53 &32.50 &38.93 &44.17 &78.53 &68.33 &73.08 &76.25 &66.12 &33.58 &44.54 &55.39 \\\cmidrule{2-18}
\multirow{20}{*}{\textbf{Encoder Decoder Models }} &mT0 &67.61 &58.41 &62.67 &65.55 &50.52 &42.18 &45.97 &48.60 &81.41 &71.47 &76.12 &79.21 &68.27 &48.54 &56.74 &63.14 \\
&mT5 &67.43 &57.30 &61.95 &65.13 &50.15 &40.81 &45.00 &47.95 &81.18 &70.71 &75.58 &78.85 &68.04 &47.79 &56.14 &62.72 \\
&AraBART &67.95 &65.62 &66.76 &67.47 &52.48 &51.84 &52.16 &52.35 &84.11 &79.02 &81.49 &83.04 &73.23 &59.94 &65.92 &70.12 \\
&AraT5 &72.41 &74.12 &73.26 &72.75 &55.95 &43.53 &48.96 &52.93 &85.46 &72.56 &78.48 &82.53 &75.23 &52.56 &61.88 &69.26 \\\cmidrule{2-18}
&"+morph" &73.30 &65.00 &68.90 &71.47 &62.63 &53.95 &57.97 &60.68 &87.02 &84.12 &85.55 &86.42 &80.37 &69.76 &74.69 &78.00 \\
&"+tokenize" &73.22 &64.92 &68.82 &71.39 &62.53 &53.96 &57.93 &60.60 &87.01 &84.52 &85.75 &86.50 &80.30 &70.48 &75.07 &78.12 \\
&"+detect" &73.20 &64.50 &68.58 &71.28 &62.45 &53.35 &57.54 &60.39 &86.94 &84.05 &85.47 &86.35 &80.23 &69.60 &74.54 &77.85 \\
&"+error" &73.38 &64.45 &68.63 &71.40 &62.58 &53.14 &57.47 &60.43 &86.99 &84.28 &85.61 &86.43 &80.22 &69.82 &74.66 &77.90 \\
&"+combined" &73.56 &64.05 &68.48 &71.44 &62.75 &52.68 &57.28 &60.44 &86.90 &83.06 &84.94 &86.10 &80.01 &67.88 &73.45 &77.25 \\\cmidrule{2-18}
&Rule Based 100k &74.13 &65.08 &69.31 &72.12 &63.33 &53.69 &58.11 &61.13 &88.09 &84.59 &86.30 &87.37 &81.56 &70.78 &75.79 &79.15 \\
&Rule Based 200k &74.22 &64.40 &68.96 &72.02 &63.26 &52.75 &57.53 &60.84 &87.94 &84.33 &86.10 &87.19 &81.06 &70.40 &75.35 &78.68 \\
&Rule Based300k &73.99 &64.22 &68.76 &71.81 &62.86 &52.42 &57.17 &60.45 &88.04 &84.47 &86.22 &87.30 &81.18 &70.54 &75.49 &78.80 \\
&Rule Based 400k &73.75 &64.79 &68.98 &71.77 &62.74 &53.26 &57.61 &60.58 &87.89 &84.74 &86.29 &87.24 &80.97 &71.10 &75.71 &78.78 \\
&Rule Based 500k &74.13 &64.66 &69.07 &72.02 &63.23 &53.12 &57.74 &60.91 &87.97 &84.71 &86.31 &87.30 &81.04 &70.96 &75.67 &78.80 \\\cmidrule{2-18}
&Corruptor 100k &73.89 &64.62 &68.94 &71.83 &63.07 &53.30 &57.77 &60.84 &87.40 &83.73 &85.53 &86.64 &80.47 &68.74 &74.14 &77.81 \\
&Corruptor 200k &74.05 &64.78 &69.11 &71.99 &63.24 &53.51 &57.97 &61.02 &87.38 &84.01 &85.66 &86.68 &80.38 &69.00 &74.26 &77.81 \\
&Corruptor 300k &74.23 &64.40 &68.97 &72.03 &63.33 &52.87 &57.63 &60.92 &87.34 &83.95 &85.61 &86.64 &80.31 &68.96 &74.20 &77.75 \\
&Corruptor 400k &74.18 &64.74 &69.14 &72.08 &63.38 &53.45 &57.99 &61.11 &87.40 &83.95 &85.64 &86.69 &80.42 &69.26 &74.42 &77.91 \\
&Corruptor 500k &74.41 &64.95 &69.36 &72.30 &63.72 &53.64 &58.25 &61.41 &87.50 &84.10 &85.77 &86.80 &80.55 &69.32 &74.51 &78.02 \\
&Corruptor 1m &74.37 &65.03 &69.39 &72.29 &63.67 &53.77 &58.30 &61.41 &87.44 &84.43 &85.91 &86.82 &80.52 &70.02 &74.90 &78.18 \\
\bottomrule
\end{tabular}}
\caption{Performance Comparison of Different Models on QALB 2015 Dataset}\label{tab:model_performance_2015}
\end{table*}

==> Tables/Areta.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccc}\toprule
\textbf{CLASS} &\textbf{GECToR\_ARBERT} &\textbf{five-shot\_2014\_expertprompt} &\textbf{five-shot\_2014-chatgpt4} &\textbf{AGEC\_million} &\textbf{rulebased\_1mill} &\textbf{AraT5 (11M)} &\textbf{COUNT} \\\midrule
OH &73.73 &89.80 &92.91 &96.34 &96.12 &87.34 &4902 \\
OT &76.59 &94.12 &95.58 &97.36 &97.07 &90.84 &708 \\
OA &78.63 &84.66 &88.93 &90.04 &89.52 &87.35 &275 \\
OW &38.57 &80.79 &86.96 &86.83 &87.50 &83.70 &107 \\
ON &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0 \\
OG &48.00 &55.74 &63.64 &63.49 &63.33 &90.32 &34 \\
OC &21.43 &28.57 &53.66 &69.57 &60.47 &87.18 &22 \\
OR &38.24 &53.02 &65.96 &74.95 &75.03 &77.10 &528 \\
OD &33.76 &51.89 &59.60 &67.35 &65.57 &73.07 &321 \\
OM &41.80 &44.53 &57.35 &73.91 &72.18 &86.44 &393 \\
OO &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0 \\
MI &11.02 &13.25 &20.53 &38.57 &32.62 &75.00 &83 \\
MT &0.00 &7.84 &11.43 &23.53 &28.57 &62.50 &7 \\
XC &32.95 &46.10 &50.78 &56.88 &58.13 &88.35 &526 \\
XF &6.06 &17.98 &23.81 &39.22 &36.00 &76.92 &29 \\
XG &37.10 &19.57 &31.35 &39.02 &40.00 &89.47 &79 \\
XN &25.19 &25.79 &31.25 &43.79 &46.33 &88.12 &108 \\
XT &3.95 &3.78 &5.48 &5.57 &5.31 &2.48 &66 \\
XM &2.04 &4.14 &6.38 &15.38 &12.24 &1.07 &26 \\
XO &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0 \\
SW &50.51 &21.25 &33.38 &54.63 &57.41 &8.29 &219 \\
SF &0.00 &6.67 &3.45 &0.00 &0.00 &57.14 &3 \\
PC &60.89 &56.25 &47.59 &53.67 &50.73 &74.98 &713 \\
PT &29.62 &29.58 &21.40 &24.04 &23.88 &57.42 &480 \\
PM &55.24 &54.21 &52.09 &47.40 &48.25 &67.08 &5599 \\
MG &25.05 &75.96 &79.70 &82.14 &81.62 &64.80 &434 \\
SP &42.27 &90.93 &91.61 &96.38 &96.70 &86.70 &805 \\\midrule
\textbf{micro avg} &55.67 &60.05 &64.51 &65.61 &65.45 &57.28 &16467 \\
\textbf{macro avg} &30.84 &39.13 &43.51 &49.63 &49.06 &61.62 &16467 \\
\textbf{weighted avg} &56.98 &66.96 &68.24 &69.99 &70.04 &76.35 &16467 \\
\bottomrule
\end{tabular}}
\caption{Performance comparison of various models on different classes of a QALB using ARETA tool}\label{tab:model_performance_comparison}
\end{table*}

==> Tables/Dataset_Error_examples.tex <==
\begin{table*}[htp]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lc}
\toprule
\textbf{Type} & \textbf{Text} \\
\midrule
\textbf{Gold Sentence }&
\begin{tabular}[l]{@{}l@{}}
\RL{ هذه ال7000 من المظاهرات خرجت بتنظيم من الأحزاب المعارضة} \\
\RL{ وسلمية ، وبدون مشاكل ، ولكن لماذا حصلت مشاكل بالمرات الأخيرة ؟} \\
\RL{وما الذي اختلف ؟ بل لأن الحكومة أرادت زرع الفتنة بين الناس وتخويفهم} \\
\RL{وإرهابهم لتفعل ما تشاء ، وتسير البلد بالديمقراطية الزائفة بل بالدكتاتورية .} \\
\RL{فمطالب الشعب لا تسمع ورميت بالمهملات ، ورأي واحد فوق رأي الجميع .}
\end{tabular} \\
\midrule
\textbf{\textbf{GPT Error Generated}} &
\begin{tabular}[l]{@{}r@{}}
\RL{هذه ال7000 من المظاهرات خرجت بتنظيم من الأحزاب المعارضة ، وسلميه} \\
\RL{، وبدون مشاكل ، ولكن ليش حصلت مشاكل بالمرات الأخيره ؟} \\
\RL{وما اللي اختلف ؟ بل لأن الحكومه ارادت زرع الفتنة بين الناس} \\
\RL{وتخويفهم وارهابهم لتفعل ما تشاء  وتسير البلد بالديمقراطيه الزائفه بالدكتاتوريه .} \\
\RL{فمطالب الشعب لا تسمع ورميت بالمهملات وروأي واحد فوق رأي الجميع .}
\end{tabular} \\
\midrule
\textbf{QALB Error} &
\begin{tabular}[l]{@{}r@{}}
\RL{هذه ال 7000 من المظاهرات خرجت بتنظيم من الاحزاب المعارضه و سلميه} \\
\RL{و بدون مشاكل و لكن لماذا حصلت مشاكل بالمرات الاخيرة و مالذي اختلف} \\
\RL{بل لان الحكومة ارادت زرع الفتنه بين الناس و تخويفهم و ارهابهم لتفعل ما تشاء} \\
\RL{و تسير البلد بالديمقراطيه الزائفه بل بالدكتاتورية فمطالب الشعب لا تسمع} \\
\RL{و رميت بالمهملات و رأي واحد فوق رأي الجميع}
\end{tabular} \\
\midrule
\textbf{Corruptor Generated} &
\begin{tabular}[l]{@{}r@{}}
\RL{من المظاهرات خرجت بتنظيم من الاحزاب المعارضة وسلمية وبدون مشاكل} \\
\RL{  ولكن لماذا حصلت مشاكل بالمرات الاخيرة وما الذي اختلف بل لان الحكومة } \\
\RL{تسير البلد بالديمقراطية الزائفة بل ارادت زرع الفتنة بين الناس وتخويفهم}  \\
\RL{فمطالب الشعب لا تسمع ورميت بالمهملات ورأي   وارهابهم لتفعل ما تشاء و } \\
\RL{واحد فوق رأي الجميع بالدكتاتورية}
\end{tabular} \\
\bottomrule
\end{tabular}}
\caption{Comparison of GPT-4, QALB and Corruptor Error Generated Texts for an Example Sentence}
\label{table:gpt_qalb_compare}
\end{table*}


==> Tables/Dataset_errorstats.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize
\begin{tabular}{lrrrrrrrr}\toprule
\textbf{Error Statistics - ChatGPT Synthetic} &\textbf{Operation} &\textbf{Count} &\textbf{\%} &\textbf{Error Statistics - Random 10,000} &\textbf{Operation} &\textbf{Count} &\textbf{\%} \\\midrule
= &No change &112069 &67.68 &= &No change &292468 &69.8 \\
| &Substitution &26035 &15.72 &| &Substitution &33891 &16.13 \\
< &insertion &14370 &8.67 &< &insertion &20227 &10.76 \\
> &deletion &2922 &1.76 &> &deletion &7125 &3.25 \\\midrule
\textbf{Error Statistics - QALB 10,000} &\textbf{Operation} &\textbf{Count} &\textbf{\%} &\textbf{Error Statistics - Corruptor 10,000} &\textbf{Operation} &\textbf{Count} &\textbf{\%} \\
= &No change &331293 &69.8 &= &No change &373538 &70.51 \\
| &Substitution &76547 &16.13 &| &Substitution &93035 &17.56 \\
< &insertion &51063 &10.76 &< &insertion &58795 &11.1 \\
> &deletion &15442 &3.25 &> &deletion &4110 &0.78 \\
\bottomrule
\end{tabular}
\caption{Error Statistics}\label{tab: error_stats}
\end{table*}

==> Tables/GEC_all.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}

\begin{table*}[!htp]\centering
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{l lccccccccccccccccc}\toprule
\multirow{2}{*}{\textbf{Settings}} &\multirow{2}{*}{\textbf{Models}} &\multicolumn{4}{c}{\textbf{Exact Match}} &\multicolumn{4}{c}{\textbf{No Alif / Ya Errors}} &\multicolumn{4}{c}{\textbf{No Punctuation}} &\multicolumn{4}{c}{\textbf{No Puncation and Alif / Ya Errors}} \\\cmidrule{3-18}
& &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} &\textbf{p} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} \\\toprule 
\multirow{3}{*}{\textbf{Baselines}} &Shared Task SOTA &73.34 &63.23 &67.91 &71.07 &64.05 &50.86 &56.70 &60.89 &85.22 &78.79 &81.88 &83.85 &80.63 &63.25 &70.89 &76.43 \\
&SOTA 2022 &79.06 &\textbf{65.79} &\textbf{71.82} &75.99 & -&- &- &- &- &- &- & & -&- &- &- \\
&Watson & -& -&\textbf{70.80} & - &- &- &- &- &- &- & -& -&- &- &- &- \\\midrule
\multirow{5}{*}{\textbf{Encoder-Decoder}} &mT0 &69.16 &52.63 &59.78 &65.07 & -&- &- &- & & -& -& -& -&- &- &- \\
&mT5 &68.99 &52.22 &59.45 &64.83 &55.66 &38.52 &45.53 &51.11 &79.85 &68.96 &74.01 &77.41 &66.47 &47.07 &55.12 &61.41 \\
&AraBART &70.71 &60.46 &65.18 &68.39 &59.04 &48.66 &53.35 &56.62 &83.42 &77.18 &80.18 &82.09 &73.08 &59.22 &65.42 &69.81 \\
&AraT5 &73.04 &63.09 &67.70 &70.81 &61.98 &51.46 &56.23 &59.55 &86.82 &83.20 &84.97 &86.07 &80.10 &68.26 &73.71 &77.41 \\
&AraT5 (AGEC-Full) &77.12 &67.85 &72.19 &75.07 &62.04 &52.69 &60.99 &62.91 &86.57 &82.70 &86.59 &87.77 &79.32 &67.19 &75.75 &77.56 \\\midrule
\multirow{4}{*}{\textbf{Encoder-Only }} &ARBERTv2 &73.89 &48.33 &58.43 &66.82 &65.94 &44.50 &53.14 &60.14 &75.52 &46.54 &57.59 &67.16 &58.58 &34.37 &43.32 &51.35 \\
&ARBERTv2 3 Stage &74.39 &47.62 &58.07 &66.87 &65.25 &41.58 &50.79 &58.58 &77.00 &46.00 &57.60 &67.85 &56.99 &28.90 &38.35 &47.71 \\
&MARBERTv2 &73.53 &48.21 &58.24 &66.54 &64.90 &43.52 &52.10 &59.09 &75.22 &45.66 &56.83 &66.60 &58.34 &35.33 &44.01 &51.62 \\
&MARBERTv2 3 Stage &74.21 &46.45 &57.14 &66.29 &65.34 &41.60 &50.83 &58.65 &76.91 &47.02 &58.36 &68.23 &57.90 &30.55 &40.00 &49.11 \\\midrule
\multirow{5}{*}{\textbf{Decoder-Only}} &LLama 7B Original &59.67 &33.84 &43.19 &51.77 &36.79 &17.69 &23.89 &30.26 &20.33 &55.56 &29.77 &23.28 &66.37 &33.15 &44.22 &55.29 \\
&Alpaca 7B &43.52 &32.55 &37.24 &40.77 &43.53 &34.64 &38.58 &41.40 &83.53 &63.60 &72.22 &78.60 &63.53 &40.89 &49.76 &57.20 \\
&Vicuna 13B &65.35 &52.65 &58.32 &62.34 &52.89 &40.45 &45.84 &49.83 &85.23 &75.24 &79.92 &83.03 &70.01 &50.46 &58.65 &64.98 \\
&bactrian-x-bloom-7b1-lora &62.33 &45.35 &52.50 &57.99 &55.24 &42.44 &48.00 &52.10 &80.89 &64.34 &71.67 &76.93 &63.53 &52.43 &57.45 &60.95 \\
&bactrian-x-llama-7b-lora &60.12 &42.90 &50.07 &55.65 &52.50 &39.53 &45.10 &49.27 &78.54 &60.50 &68.35 &74.12 &60.11 &49.54 &54.32 &57.65 \\\midrule
\multirow{3}{*}{\textbf{ChatGPT}} &ChatGPT -1 &58.71 &49.29 &53.59 &56.55 &46.69 &40.82 &43.56 &45.38 &59.81 &64.35 &62.00 &60.67 &41.55 &53.80 &46.89 &43.53 \\
&ChatGPT -3 &64.60 &60.37 &62.41 &63.71 &54.06 &52.51 &53.28 &53.74 &66.09 &70.88 &68.40 &67.00 &48.14 &58.78 &52.93 &49.95 \\
&ChatGPT -5 &64.70 &59.59 &62.04 &63.61 &54.01 &51.28 &52.61 &53.44 &66.33 &70.80 &68.49 &67.18 &48.63 &58.48 &53.10 &50.33 \\\midrule
\multirow{3}{*}{\textbf{ChatGPT-EP}} &ChatGPT EP - 1 &60.49 &51.37 &55.56 &58.42 &48.70 &42.86 &45.59 &47.41 &62.07 &65.86 &63.91 &62.79 &43.52 &54.60 &48.44 &45.36 \\
&ChatGPT EP - 3 &65.83 &61.41 &63.54 &64.90 &55.54 &53.54 &54.52 &55.13 &67.50 &71.52 &69.45 &68.27 &50.17 &59.10 &54.27 &51.73 \\
&ChatGPT EP - 5 &66.53 &61.62 &63.98 &65.49 &56.56 &54.11 &55.31 &56.05 &68.49 &71.61 &70.02 &69.09 &51.69 &59.84 &55.47 &53.14 \\\midrule
\multirow{2}{*}{\textbf{GPT-4}} &ChatGPT4 - 3shot &69.31 &59.24 &63.88 &67.03 & 57.79& 48.12& 52.51 & 55.55&74.43 &78.11 & 76.23& 75.31&60.60 &66.19 &62.97 &61.64\\
&ChatGPT4 - 5shot &69.46 &61.96 &65.49 &67.82 & 58.44& 51.47&54.73 &56.89 &74.59 &78.15 &76.33 & 75.27&60.06 & 65.75& 62.78& 61.17\\
\toprule
\end{tabular}}
\caption{Comprehensive Evaluation of NLP Models across Various Configurations and Error Handling Scenarios, Highlighting Precision, Recall, and F1 Scores}\label{tab: GEC_all}
\end{table*}


%\begin{table*}[!htp]
%\centering
%\scriptsize
%\resizebox{\textwidth}{!}{
%\begin{tabular}{l lcccccccc}
%\toprule
%\multirow{2}{*}{\textbf{Settings}} & \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{QALB-2014}} & \multicolumn{2}{c}{\textbf{QALB-2015}} \\
%\cmidrule(lr){3-4} \cmidrule(lr){5-6}
%& & \textbf{P} & \textbf{R} & \textbf{P} & \textbf{R} \\
%\toprule
%\multirow{5}{*}{\textbf{Encoder-Decoder}} & mT0 & 69.16 & 52.63 & - & - \\
%& mT5 & 68.99 & 52.22 & 79.85 & 68.96 \\
%& AraBART & 70.71 & 60.46 & 83.42 & 77.18 \\
%& AraT5 & 73.04 & 63.09 & 86.82 & 83.20 \\
%& AraT5 (AGEC-Full) & 77.12 & 67.85 & 86.57 & 82.70 \\
%\midrule
%\multirow{4}{*}{\textbf{Encoder-Only}} & ARBERTv2 & 73.89 & 48.33 & 75.52 & 46.54 \\
%& ARBERTv2 3 Stage & 74.39 & 47.62 & 77.00 & 46.00 \\
%& MARBERTv2 & 73.53 & 48.21 & 75.22 & 45.66 \\
%& MARBERTv2 3 Stage & 74.21 & 46.45 & 76.91 & 47.02 \\
%\midrule
%\multirow{5}{*}{\textbf{Decoder-Only}} & LLama 7B Original & 59.67 & 33.84 & 20.33 & 55.56 \\
%& Alpaca 7B & 43.52 & 32.55 & 83.53 & 63.60 \\
%& Vicuna 13B & 65.35 & 52.65 & 85.23 & 75.24 \\
%& bactrian-x-bloom-7b1-lora & 62.33 & 45.35 & 80.89 & 64.34 \\
%& bactrian-x-llama-7b-lora & 60.12 & 42.90 & 78.54 & 60.50 \\
%\midrule
%\multirow{3}{*}{\textbf{ChatGPT}} & ChatGPT -1 & 58.71 & 49.29 & 59.81 & 64.35 \\
%& ChatGPT -3 & 64.60 & 60.37 & 66.09 & 70.88 \\
%& ChatGPT -5 & 64.70 & 59.59 & 66.33 & 70.80 \\
%\midrule
%\multirow{3}{*}{\textbf{ChatGPT-EP}} & ChatGPT EP - 1 & 60.49 & 51.37 & 62.07 & 65.86 \\
%& ChatGPT EP - 3 & 65.83 & 61.41 & 67.50 & 71.52 \\
%& ChatGPT EP - 5 & 66.53 & 61.62 & 68.49 & 71.61 \\
%\midrule
%\multirow{2}{*}{\textbf{GPT-4}} & ChatGPT4 - 3shot & 69.31 & 59.24 & 74.43 & 78.11 \\
%& ChatGPT4 - 5shot & 69.46 & 61.96 & 74.59 & 78.15 \\
%\bottomrule
%\end{tabular}
%}
%\caption{Comprehensive Evaluation of NLP Models: Exact Match and No Punctuation}
%\label{tab:GEC_all}
%\end{table*}


==> Tables/GEC_results_v2.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
% \begin{landscape}
\begin{table*}[!htp]\centering
\scriptsize
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|r|rrrr|rrrr|rrrr|rrrr|}\toprule
\multirow{2}{*}{\textbf{Settings}} &\multirow{2}{*}{\textbf{Models}} &\multicolumn{4}{c}{\textbf{Exact Match}} &\multicolumn{4}{c}{\textbf{No Alif / Ya Errors}} &\multicolumn{4}{c}{\textbf{No Punctuation}} &\multicolumn{4}{c}{\textbf{No Puncation and Alif / Ya Errors}} \\\cmidrule{3-18}
& &\textbf{P} &\textbf{R} &\textbf{F\_1.0 } &\textbf{F\_0.5} &\textbf{P} &\textbf{R} &\textbf{F\_1.0 } &\textbf{F\_0.5} &\textbf{P} &\textbf{R} &\textbf{F\_1.0 } &\textbf{F\_0.5} &\textbf{p} &\textbf{R} &\textbf{F\_1.0 } &\textbf{F\_0.5} \\\midrule
\multirow{3}{*}{Official Baselines} &Shared Task SOTA &73.34 &63.23 &67.91 &71.07 &64.05 &50.86 &56.7 &60.89 &85.22 &78.79 &81.88 &83.85 &80.63 &63.25 &70.89 &76.43 \\
&SOTA 2022 &79.06 &\textbf{65.79} &\textbf{71.82} &75.99 & & & & & & & & & & & & \\
&Watson & & &\textbf{70.8} & & & & & & & & & & & & & \\\midrule
\multirow{4}{*}{Encoder-Decoder Baselines} &mT0 &69.16 &52.63 &59.78 &65.07 &55.88 &38.86 &45.84 & & $80.00$&$69.78$ & $74.54$& &$67.16$ &$48.27$ &$56.17$ & \\
&mT5 &68.99 &52.22 &59.45 &64.83 &55.66 &38.52 &45.53 &51.11 &79.85 &68.96 &74.01 &77.41 &66.47 &47.07 &55.12 &61.41 \\
&AraBART &70.71 &60.46 &65.18 &68.39 &59.04 &48.66 &53.35 &56.62 &83.42 &77.18 &80.18 &82.09 &73.08 &59.22 &65.42 &69.81 \\
&AraT5x &73.04 &63.09 &67.7 &70.81 &61.98 &51.46 &56.23 &59.55 &86.82 &83.2 &84.97 &86.07 &80.1 &68.26 &73.71 &77.41 \\\midrule
\multirow{4}{*}{Encoder-Decoder Experiments} &AraT5x (100,000) - AGEC original &73.39 &64.12 &68.44 &71.33 &62.34 &54.66 &58.25 &60.64 &86.72 &83.58 &85.12 &86.07 &79.68 &68.82 &73.85 &77.24 \\
&AraT5x (100,000) - Gold/generated &73.68 &63.85 &68.42 &71.48 &62.81 &52.39 &57.13 &60.41 &86.98 &83.11 &85 &86.18 &80.06 &67.9 &73.48 &77.29 \\
&AraT5x (100,0000 - AGEC/generated &73.16 &63.77 &68.15 & &62.13 &52.14 &56.70 & &86.95 &83.57 &85.22 & &80.12 &68.68 &73.96 & \\
&\hl{AraT5x (AGEC-Full)} &72.89 &64.01 &\hl{\textbf{72.19}?} &70.92 &62.04 &52.69 &56.99 &59.91 &86.57 &82.7 &84.59 &85.77 &79.32 &67.19 &72.75 &76.56 \\\midrule
\multirow{4}{*}{Encoder-Only } &Gector- ARBERv2 Backbone &73.89 &48.33 &58.43 &66.82 &65.94 &44.5 &53.14 &60.14 &75.52 &46.54 &57.59 &67.16 &58.58 &34.37 &43.32 &51.35 \\
&Gector - ARBERTv2 Backbone 3 step training &74.39 &47.62 &58.07 &66.87 &65.25 &41.58 &50.79 &58.58 &77 &46 &57.6 &67.85 &56.99 &28.9 &38.35 &47.71 \\
&Gector - MARBERTv2 Backbone &73.53 &48.21 &58.24 &66.54 & & & & & & & & & & & & \\
&Gector - MARBERTv2 Backbone 3 step training &74.21 &46.45 &57.14 &66.29 & & & & & & & & & & & & \\\midrule
\multirow{5}{*}{Decoder-Only} &LLama 7B Original &59.67 &33.84 &43.19 &51.77 &36.79 &17.69 &23.89 &30.26 &20.33 &55.56 &29.77 &23.28 &66.37 &33.15 &44.22 &55.29 \\
&Alpaca 7B &43.52 &32.55 &37.24 &40.77 &43.53 &34.64 &38.58 &41.40 &83.53 &63.6 &72.22 &78.60 &63.53 &40.89 &49.76 &57.20 \\
&Vicuna 13B &65.35 &52.65 &58.32 &62.34 &52.89 &40.45 &45.84 &49.83 &85.23 &75.24 &79.92 &83.03 &70.01 &50.46 &58.65 &64.98 \\
&MBZUAI/bactrian-x-bloom-7b1-lora &62.33 &45.35 &52.50 &57.99 &55.24 &42.44 &48.00 &52.10 &80.89 &64.34 &71.67 &76.93 &63.53 &52.43 &57.45 &60.95 \\
&MBZUAI/bactrian-x-llama-7b-lora &60.12 &42.9 &50.07 &55.65 &52.5 &39.53 &45.10 &49.27 &78.54 &60.5 &68.35 &74.12 &60.11 &49.54 &54.32 &57.65 \\\midrule
\multirow{3}{*}{ChatGPT} &ChatGPT -1 &58.71 &49.29 &53.59 &56.55 &46.69 &40.82 &43.56 &45.38 &59.81 &64.35 &62.00 &60.67 &41.55 &53.8 &46.89 &43.53 \\
&ChatGPT -3 &64.60 &60.37 &62.41 &63.71 &54.06 &52.51 &53.28 &53.74 &66.09 &70.88 &68.4 &67.00 &48.14 &58.78 &52.93 &49.95 \\
&ChatGPT -5 &64.7 &59.59 &62.04 &63.61 &54.01 &51.28 &52.61 &53.44 &66.33 &70.8 &68.49 &67.18 &48.63 &58.48 &53.1 &50.33 \\\midrule
\multirow{3}{*}{ChatGPT-EP} &ChatGPT EP - 1 &60.49 &51.37 &55.56 &58.42 &48.70 &42.86 &45.59 &47.41 &62.07 &65.86 &63.91 &62.79 &43.52 &54.6 &48.44 &45.36 \\
&ChatGPT EP - 3 &65.83 &61.41 &63.54 &64.90 &55.54 &53.54 &54.52 &55.13 &67.50 &71.52 &69.45 &68.27 &50.17 &59.1 &54.27 &51.73 \\
&ChatGPT EP - 5 &66.53 &61.62 &63.98 &65.49 &56.56 &54.11 &55.31 &56.05 &68.49 &71.61 &70.02 &69.09 &51.69 &59.84 &55.47 &53.14 \\\midrule
\multirow{2}{*}{GPT-4} &ChatGPT4 - 3shot &69.31 &59.24 &63.88 &67.03 &57.79 &48.12 &52.51 & & 74.43&78.11 &76.23& &60.60 &66.19 &62.97 & \\
&ChatGPT4 - 5shot &69.46 &61.96 &65.49 &67.82 & 58.44& 51.47& 54.73& & 74.59& 78.15& 76.33& & 60.06& 65.75& 62.78& \\
\bottomrule
\end{tabular}}
\caption{Comparison of Various Models' Performances in Different Settings, Including Baselines, Encoder-Decoder Experiments, Encoder-Only, Decoder-Only, ChatGPT, ChatGPT-EP, and GPT-4. The metrics used for evaluation are Precision (P), Recall (R), F1-Score (F\_1.0), and F0.5-Score (F\_0.5) under conditions of Exact Match, No Alif/Ya Errors, No Punctuation, and No Punctuation and Alif/Ya Errors.}\label{tab: comparison}
\end{table*}
% \end{landscape}


==> Tables/GED_results.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\scriptsize
\resizebox{\linewidth}{!}{
\begin{tabular}{lcrrrrr}\toprule
\textbf{Models} &\textbf{Number}\textbf{ of} \textbf{classes} &\textbf{P }&\textbf{R} & \textbf{F}\textsubscript{1} &\textbf{Accuracy} \\\toprule
\multirow{2}{*}{\textbf{ARBERTv2}} &2 &65.56 &59.45 &62.35 &84.32 \\
&7 &61.84 &56.59 &59.10 &85.77 \\\midrule
\multirow{2}{*}{\textbf{MARBERTv2}} &2 &58.71 &54.24 &56.39 &80.34 \\
&7 &56.54 &49.53 &52.80 &81.34 \\
\bottomrule
\end{tabular}}
\caption{Comparative evaluation of ARBERTv2 and MARBERTv2 models in grammar error detection tasks.}\label{Table:GED}
\end{table}

==> Tables/GPT_corruptor.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrrrr}\toprule
\multirow{2}{*}{\textbf{Settings}} &\multirow{2}{*}{\textbf{Models}} &\multicolumn{4}{c}{\textbf{Exact Match}} \\\cmidrule{3-6}
& &\textbf{P} &\textbf{R} &\textbf{F\_1.0 } &\textbf{F\_0.5} \\\midrule
\multirow{5}{*}{\textbf{Synthetic Data - ChatGPT}} &GPT - Synthetic Data (10,000) &73.69 &61.42 &67 &70.86 \\
&\textbf{QALB 10,000} &73.22 &64.06 &68.33 &71.18 \\
&Corruptor 10,000 ( QALB examples) &72.47 &58.13 &64.51 &69.06 \\
&Corruptor 10,000 ( Random examples) &63.69 &30.35 &41.1 &52.22 \\
&Combined &73.08 &64.26 &68.39 &71.13 \\ \bottomrule
\end{tabular}}
\caption{Synthetic Data - ChatGPT}\label{tab: synth_chat}
\end{table*}

==> Tables/Gector_tags.tex <==
\begin{table}[ht]
\centering
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{lr}
\toprule
\textbf{Operation} & \textbf{Count} \\
\midrule
KEEP & 725553 \\
REPLACE & 201920 \\
APPEND & 75157 \\
DELETE & 13555 \\
MERGE & 5703 \\
\bottomrule
\end{tabular}%
}
\caption{Count of each operation in the tag vocabulary.}
\label{tab:operation_count}
\end{table}


==> Tables/New_results.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|r|rrrrrrrrrrrrr}\toprule
\multirow{2}{*}{\textbf{Settings}} &\multirow{2}{*}{\textbf{Models}} &\multicolumn{3}{c}{\textbf{Exact Match}} &\multicolumn{3}{c}{\textbf{No Alif / Ya Errors}} &\multicolumn{3}{c}{\textbf{No Punctuation}} &\multicolumn{3}{c}{\textbf{No Puncation and Alif / Ya Errors}} \\\cmidrule{3-14}
& &\textbf{P} &\textbf{R} &\textbf{F\_1.0 } &\textbf{P} &\textbf{R} &\textbf{F\_1.0 } &\textbf{P} &\textbf{R} &\textbf{F\_1.0 } &\textbf{P} &\textbf{R} &\textbf{F\_1.0 } \\\midrule
\multirow{2}{*}{\textbf{Baselines}} &\textbf{Shared Task SOTA} &73.34 &63.23 &67.91 &83.34 &50.86 &56.7 &85.22 &78.79 &81.88 &80.63 &63.25 &70.89 \\
&\textbf{S+ (2022)} &\textbf{79.06} &\textbf{65.79} &\textbf{71.82} &\textbf{} &\textbf{} &\textbf{} &\textbf{} &\textbf{} &\textbf{} &\textbf{} &\textbf{} &\textbf{} \\\hline
\multirow{5}{*}{\textbf{Encoder Decoder Models }} &\textbf{mt5-base} &68.53 &52.78 &59.64 &55.34 &39.43 &46.05 &79.15 &68.44 &73.41 &64.83 &46.49 &54.15 \\
&\textbf{mt0-base} &68.81 &52.99 &59.87 &55.64 &39.56 &46.25 &79.51 &69.22 &74.01 &65.97 &47.61 &55.31 \\
&\textbf{AraBART} &70.03 &61 &65.2 &58.46 &49.47 &53.59 &83.01 &76.82 &79.8 &72.09 &58.46 &64.56 \\
&\textbf{AraT5xV2 } &72.65 &65.76 &69.03 &62.54 &54.65 &58.33 &86.90 &83.44 &85.13 &79.05 &67.43 &72.78 \\
&\textbf{AraT5xV2 Synthetic Data} &\textbf{78.02} &\textbf{65.55} &\textbf{71.24} &\textbf{72.1} &\textbf{66.667} &\textbf{69.28} &\textbf{90.01} &\textbf{84.6} &\textbf{87.22} &\textbf{84.9} &\textbf{72.2} &\textbf{78.04} \\\hline
\multirow{6}{*}{\textbf{GEC Instrctions }} &\textbf{Bloomz 7B} &68.91 &55.53 &61.50 &56.35 &40.65 &47.23 &80.53 &71.33 &75.65 &66.45 &50.92 &57.66 \\
&\textbf{LLama 7B Original} &59.67 &33.84 &43.19 &36.79 &17.69 &23.89 &20.33 &55.56 &29.77 &66.37 &33.15 &44.22 \\
&\textbf{Alpaca 7B } &43.52 &32.55 &37.24 &43.53 &34.64 &38.58 &83.53 &63.6 &72.22 &63.53 &40.89 &49.76 \\
&\textbf{Vicuna 13B} &65.35 &52.65 &58.32 &52.89 &40.45 &45.84 &85.23 &75.24 &79.92 &70.01 &50.46 &58.65 \\
&\textbf{bactrian-x-bloom} &62.33 &45.35 &52.50 &55.24 &42.44 &48.00 &80.89 &64.34 &71.67 &63.53 &52.43 &57.45 \\
&\textbf{bactrian-x-llama} &60.12 &42.9 &50.07 &52.5 &39.53 &45.10 &78.54 &60.5 &68.35 &60.11 &49.54 &54.32 \\\hline
\multirow{3}{*}{\textbf{ChatGPT}} &\textbf{ChatGPT 1-Shot} &58.71 &49.29 &53.59 &46.69 &40.82 &43.56 &59.81 &64.35 &62 &41.55 &53.8 &46.89 \\
&\textbf{ChatGPT 3-Shot} &64.6 &60.37 &62.41 &54.06 &52.51 &53.28 &66.09 &70.88 &68.4 &48.14 &58.78 &52.93 \\
&\textbf{ChatGPT 5-Shot} &64.7 &59.59 &62.04 &54.01 &51.28 &52.61 &66.33 &70.8 &68.49 &48.63 &58.48 &53.1 \\
\bottomrule
\end{tabular}
}
\caption{Compartive table For QALB 2014 (TBD)}\label{tab: }
\end{table*}

==> Tables/New_results2.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\scriptsize
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|r|rrrrrrrrrrrrr}\toprule
\multirow{2}{*}{\textbf{Settings}} &\multirow{2}{*}{\textbf{Models}} &\multicolumn{3}{c}{\textbf{Exact Match}} &\multicolumn{3}{c}{\textbf{No Alif / Ya Errors}} &\multicolumn{3}{c}{\textbf{No Punctuation}} &\multicolumn{3}{c}{\textbf{No Puncation and Alif / Ya Errors}} \\\cmidrule{3-14}
& &\textbf{P} &\textbf{R} &\textbf{F\_1.0 } &\textbf{P} &\textbf{R} &\textbf{F\_1.0 } &\textbf{P} &\textbf{R} &\textbf{F\_1.0 } &\textbf{P} &\textbf{R} &\textbf{F\_1.0 } \\\midrule
\multirow{2}{*}{\textbf{Baselines}} &\textbf{Shared Task SOTA} &73.34 &63.23 &67.91 &83.34 &50.86 &56.7 &85.22 &78.79 &81.88 &80.63 &63.25 &70.89 \\
&\textbf{S+ (2022)} &\textbf{78.36} &\textbf{70.43} &\textbf{74.18} &\textbf{} &\textbf{} &\textbf{} &\textbf{} &\textbf{} &\textbf{} &\textbf{} &\textbf{} &\textbf{} \\\hline
\multirow{6}{*}{\textbf{Encoder Decoder Models }} &\textbf{AraBART} &67.95 &65.62 &66.76 &52.48 &51.84 &52.16 &84.11 &79.02 &81.49 &73.23 &59.94 &65.92 \\
&\textbf{AraT5x} &71.31 &\textbf{73.48} &\textbf{72.38} & & & & & & & & & \\
&\textbf{mT0} &67.61 &58.41 &62.67 &50.52 &42.18 &45.97 &81.41 &71.47 &76.12 &68.27 &48.54 &56.74 \\
&\textbf{mT5} &67.43 &57.3 &61.95 &50.15 &40.81 &45 &81.18 &70.71 &75.58 &68.04 &47.79 &56.15 \\
&\textbf{AraT5xV2 } &72.41 &74.12 &73.26 &55.95 &43.53 &48.96 &85.46 &72.56 &78.48 &75.23 &52.56 &61.88 \\
&\textbf{AraT5xV2 Synthetic Data} &\textbf{76.9} &\textbf{74.96} &\textbf{75.92} &\textbf{57.35} &\textbf{45.66} &\textbf{50.84} &\textbf{86.93} &\textbf{73.89} &\textbf{79.88} &\textbf{76.22} &\textbf{55.58} &\textbf{64.28} \\\hline
\multirow{6}{*}{\textbf{GEC Instrctions }} &\textbf{Bloomz 7B} &64.4 &62.64 &63.51 &49.5 &38.5 &43.31 &79.24 &69.57 &74.09 &69.25 &39.8 &50.55 \\
&\textbf{LLama 7B Original} &59.59 &38.72 &46.94 &34.4 &20.55 &25.73 &72.46 &56.88 &67.17 &69.01 &35.77 &47.12 \\
&\textbf{Alpaca 7B } &50.24 &32.42 &39.41 &32.3 &19.23 &24.11 &70.34 &66.67 &68.46 &66.88 &32.5 &43.74 \\
&\textbf{Vicuna 13B} &62.53 &40.9 &49.45 &35.55 &21.5 &26.79 &75.46 &69.56 &72.39 &67.33 &35.33 &46.34 \\
&\textbf{MBZUAI/bactrian-x-bloom-7b1-lora} &65.46 &42.53 &51.56 &52.35 &39.4 &44.96 &80.01 &70.45 &74.93 &69.55 &36.88 &48.20 \\
&\textbf{MBZUAI/bactrian-x-llama-7b-lora} &58.35 &40.24 &47.63 &48.53 &32.5 &38.93 &78.53 &68.33 &73.08 &66.12 &33.58 &44.54 \\\hline
\multirow{3}{*}{\textbf{ChatGPT}} &\textbf{ChatGPT 1-Shot} &49.82 &46.72 &48.22 &34.89 &38 &36.38 &52.69 &60.68 &56.4 &33.17 &50.84 &40.15 \\
&\textbf{ChatGPT 3-Shot} &52.33 &47.57 &49.83 &37.93 &39.97 &38.92 &53.38 &56.63 &54.96 &33.33 &46.77 &38.92 \\
&\textbf{ChatGPT 5-Shot} &\textbf{-} &\textbf{-} &\textbf{-} &\textbf{-} &\textbf{-} &\textbf{-} &\textbf{-} &\textbf{-} &\textbf{-} &\textbf{-} &\textbf{-} &\textbf{-} \\
\bottomrule
\end{tabular}}
\end{table*}

==> Tables/Qalb_error_types.tex <==
\begin{table}[h!]
\centering
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
 & \textbf{Edit} & \textbf{Add} & \textbf{Merge} & \textbf{Split} & \textbf{Delete} & \textbf{Move} & \textbf{Other} & \textbf{Domain} \\
\midrule
\textbf{Train} & 55.34 & 32.36 & 5.95 & 3.48 & 2.21 & 0.14 & 0.50 & Comments\\
\textbf{Dev} & 53.51 & 34.24 & 5.97 & 3.67 & 2.03 & 0.08 & 0.49 & Comments\\
\textbf{Test} & 51.94 & 34.73 & 5.89 & 3.48 & 3.32 & 0.15 & 0.49 & Comments\\
\bottomrule
\end{tabular}}
\caption{Percentage of error types for QALB-2014 data splits.}
\label{tab:DataErrorTypePercentages}
\end{table}


==> Tables/corrupt_format.tex <==
\begin{table*}[]
\centering
\scriptsize
\resizebox{0.90\columnwidth}{!}{
\begin{tabular}{lr}
\toprule
~~~~~~~~~ \textbf{Fine-tune Instruction Example} \\
\toprule
You are an AI model that introduces grammatical errors into Arabic text. These errors can span across orthography, morphology, syntax, semantics, punctuation, and word segmentation. \\
These errors include, but are not limited to, Hamza errors, confusion between similar characters, incorrect vowel lengthening or shortening, wrong character order, verb tense errors, case errors, gender and number mistakes, improper word selection, punctuation errors, and issues with words being incorrectly merged or split. \\
Take a correctly written sentence and modify it to contain some of these errors. \\
You operate on sentences labeled \textit{<input> SRC </input>}, correcting them into their ideal form, labeled as \textit{<output> TGT </output>}. \\
\colorbox{blue!25}{\#\#\# Instruction:} \\
Please introduce grammatical errors into the following sentence indicated by \textit{<input> SRC </input>} tag. You need to comprehend the sentence as a whole before gradually introducing errors while keeping the original sentence structure unchanged as much as possible. \\
Afterward, output the modified version directly without any explanations. Please feel free to refer to this example. Remember to format your modified output results with the tag \textit{<output> Your Modified Version </output>}. Please start: \textit{<input> {text} </input>}. \\
\bottomrule
\end{tabular}
}
\caption{Modified data format for the LLaMA instruction fine-tuning step.}\label{tab:corrupt_prompt}
\end{table*}


==> Tables/gpt4_explain.tex <==
\begin{table*}[!htp]\centering
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{lllll}\toprule
Task &Predicted &Reference &GPT4 &Explanation \\\midrule
Error Correction &
\begin{tabular}[c]{@{}l@{}}
\RL{أدعو وبكل الحاح رجال الأعمال العرب}\\
\RL{ودو ل مجلس التعاون في الخليج العربي}\\
\RL{إلى انتهاز الفرصةوالإستثمار بتونس}\\
\RL{بكيفيةمكث فة ، وإذا توف ر ذلك بقيمة محترمة}\\
\RL{من قطر والإمارات والسعودية والكويت}\\
\RL{ورجال أعمال كل هذه الدو ل}\\
\RL{سنصل إن شاء الله إلى نسبة نمو}\\
\RL{لا تقل عن عشرة في المائة}\\
\RL{إن لم يكن أكثر٠}
\end{tabular}&
\begin{tabular}[c]{@{}l@{}}
\RL{أدعو وبكل إلحاح رجال الأعمال العرب}\\
\RL{ودول مجلس التعاون في الخليج العربي}\\
\RL{إلى انتهاز الفرصة والإستثمار بتونس}\\
\RL{بكيفية مكثفة . وإذا توفر ذلك بقيمة محترمة}\\
\RL{من قطر ، والإمارات ، والسعودية ، والكويت}\\
\RL{ورجال أعمال كل هذه الدول}\\
\RL{سنصل إن شاء الله إلى نسبة نمو}\\
\RL{لا تقل عن عشرة في المائة}\\
\RL{إن لم يكن أكثر .}
\end{tabular}&
\begin{tabular}[c]{@{}l@{}}
\RL{أدعو بكل الحاح رجال الأعمال العرب}\\
\RL{ودول مجلس التعاون في الخليج العربي}\\
\RL{إلى انتهاز الفرصة والاستثمار بتونس}\\
\RL{بكيفية مكثفة. وإذا توفر ذلك بقيمة محترمة}\\
\RL{من قطر والإمارات والسعودية والكويت}\\
\RL{ورجال أعمال كل هذه الدول}\\
\RL{سنصل إن شاء الله إلى نسبة نمو}\\
\RL{لا تقل عن عشرة في المائة}\\
\RL{إن لم يكن أكثر.}
\end{tabular}& 
\begin{tabular}[c]{@{}l@{}}
1. \RL{“دو ل”} corrected to \RL{“دول”} \\ for the proper word for “countries” in Arabic.\\
2. \RL{“الفرصةوالإستثمار”} corrected to \RL{“الفرصة والاستثمار”} \\
for proper spacing and removed  \\
the unnecessary diacritic on the word \\
3.\RL{“بكيفيةمكث فة”} corrected to \RL{“بكيفية مكثفة”}\\ for proper spacing and meaningful sentence.\\
4. \RL{“توف ر”} corrected to \RL{“توفر”}\\ for the correct word “provided”. 
\end{tabular} \\
\midrule
Error Detection &
\begin{tabular}[c]{@{}l@{}}
\RL{أدعو وبكل الحاح رجال الأعمال العرب}\\
\RL{ودو ل مجلس التعاون في الخليج العربي}\\
\RL{إلى انتهاز الفرصةوالإستثمار بتونس}\\
\RL{بكيفيةمكث فة ، وإذا توف ر ذلك بقيمة محترمة}\\
\RL{من قطر والإمارات والسعودية والكويت}\\
\RL{ورجال أعمال كل هذه الدو ل}\\
\RL{سنصل إن شاء الله إلى نسبة نمو}\\
\RL{لا تقل عن عشرة في المائة}\\
\RL{إن لم يكن أكثر٠}
\end{tabular}&
\begin{tabular}[c]{@{}l@{}}
\RL{أدعو وبكل إلحاح رجال الأعمال العرب}\\
\RL{ودول مجلس التعاون في الخليج العربي}\\
\RL{إلى انتهاز الفرصة والإستثمار بتونس}\\
\RL{بكيفية مكثفة . وإذا توفر ذلك بقيمة محترمة}\\
\RL{من قطر ، والإمارات ، والسعودية ، والكويت}\\
\RL{ورجال أعمال كل هذه الدول}\\
\RL{سنصل إن شاء الله إلى نسبة نمو}\\
\RL{لا تقل عن عشرة في المائة}\\
\RL{إن لم يكن أكثر .}
\end{tabular}&
\begin{tabular}[c]{@{}l@{}}
\RL{أدعو وبكل الحاح رجال الأعمال العرب}\\
\RL{ودول مجلس التعاون في الخليج العربي}\\
\RL{إلى انتهاز الفرصة والاستثمار بتونس}\\
\RL{بكيفية مكثفة، وإذا توفر ذلك بقيمة محترمة}\\
\RL{من قطر والإمارات والسعودية والكويت}\\
\RL{ورجال أعمال كل هذه الدول}\\
\RL{سنصل إن شاء الله إلى نسبة نمو}\\
\RL{لا تقل عن عشرة في المائة}\\
\RL{إن لم يكن أكثر.}
\end{tabular}& 
\begin{tabular}[c]{@{}l@{}}
1. \RL{'دو ل ← دول'} ||| SP \\
2.\RL{‘الفرصةوالإستثمار ← الفرصة والاستثمار’} ||| SP \\
3. \RL{‘بكيفيةمكث فة ← بكيفية مكثفة’} ||| SP \\
4.\RL{‘توف ر ← توفر’} ||| SP \\
5.\RL{‘الدو ل ← الدول’} ||| SP 
\end{tabular} \\
\bottomrule
\end{tabular}}
\caption{Analysis of GPT-4's performance in error detection and correction in Arabic text. The tables present the original text, the reference corrected text, and the outcome from GPT-4, along with detailed explanations of each detected and corrected error.}\label{tab:gpt4_explain}
\end{table*}


==> Tables/hyperparamerts_gen.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\scriptsize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr|rrrrr}\toprule
\textbf{Decoding Method} &\multicolumn{4}{c}{\textbf{QALB-2014}} &\multicolumn{4}{c}{\textbf{QALB-2015}} \\\cmidrule{1-9}
\textbf{AraT5\textsubscript{v2} (11M)} &\textbf{P} &\textbf{R} &\textbf{F1} &\textbf{F0.5} &\textbf{P} &\textbf{R} &\textbf{F1} &\textbf{F0.5} \\\midrule
\textbf{Greedy} &74.64 &66.3 &70.22 &72.81 &67.63 &67.84 &67.74 &67.68 \\
\textbf{Beam} &76.51 &69.92 &73.07 &75.09 &70.13 &67.92 &69.01 &69.68 \\
\textbf{Top-p} &77.12 &69.83 &73.29 &75.54 &72.41 &74.12 &73.26 &72.75 \\
\bottomrule
\end{tabular}}
\caption{Impact of different decoding methods on model performance}\label{tab: hyper_gen}
\end{table}

==> Tables/line_graph.tex <==
\begin{figure*}
     \centering
% First row with two images
\begin{subfigure}{0.47\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Images/2014_2.png}
    \caption{Tested on QALB-2014 }
    \label{fig:2014_line}
\end{subfigure}
\begin{subfigure}{0.98\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{Images/2015_2.png}
    \caption{Tested on QALB-2015 L1}
    \label{fig:2015_line}
\end{subfigure}

\caption{F1 scores for systems trained on 100k to 1m sentences of parallel data}
\label{fig:line_graph}
\end{figure*}


==> Tables/multitask.tex <==
\begin{table}[]\centering
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llcccc|cccc}\toprule
\multirow{2}{*}{\textbf{Settings}} &\multirow{2}{*}{\textbf{Models}} &\multicolumn{4}{c}{\textbf{QALB-2014}} &\multicolumn{4}{c}{\textbf{QALB-2015}}\\\cmidrule{3-6}\cmidrule{7-10}
& &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}}\\ \toprule 
\multirow{1}{*}{\textbf{Baselines}} 
&AraT5 &$\mathbf{73.04}$ &$63.09$ &$67.70$ &$70.81$ &$\mathbf{72.41}$ &$\mathbf{74.12}$ &$\mathbf{73.26}$ &$\mathbf{72.75}$\\
\midrule
\multirow{4}{*}{\textbf{Auxiliary Tasks}} 
&+ Translate &$72.98$ &$63.93$ &$68.16$ &$70.97$ &$71.82$ &$71.86$ &$71.84$ &$71.82$\\
&+ Transliterate &$72.63$ &$65.53$ &$68.79$ &$71.08$ &$71.10$ &$72.07$ &$71.58$ &$71.29$\\
&+ Diacritize &$72.86$ &$64.90$ &$68.65$ &$71.11$ &$70.87$ &$72.41$ &$71.63$ &$71.17$\\
&+ All Combined &$73.06$ &$64.64$ &$68.59$ &$\mathbf{71.20}$ &$71.47$ &$72.26$ &$71.86$ &$71.62$\\
\midrule
\multirow{2}{*}{\textbf{Morphological Disambiguator}} 
&+ Morphology &$72.57$ &$66.14$ &$69.21$ &$71.18$ &$70.87$ &$72.76$ &$71.81$ &$71.24$\\
&+ Tokenize &$72.73$ &$64.70$ &$68.48$ &$70.96$ &$71.28$ &$71.79$ &$71.53$ &$71.38$\\
\midrule
\multirow{2}{*}{\textbf{GED}} 
&+ Error &$72.96$ &$65.11$ &$68.81$ &$71.24$ &$71.23$ &$72.12$ &$71.67$ &$71.40$\\
&+ Detect &$72.76$ &$64.97$ &$68.65$ &$71.05$ &$71.51$ &$72.10$ &$71.80$ &$71.62$\\
\midrule
\multirow{1}{*}{\textbf{All combined}}
&+ All Combined &$72.26$ &$\mathbf{66.49}$ & $\mathbf{69.25}$ &$71.02$ &$70.63$ &$73.46$ &$72.01$ &$71.17$\\
\toprule
\end{tabular}}
\caption{Multitask Results for QALB 2014 and 2015 } \label{tab:multitask_full}
\end{table}


==> Tables/seq2seq_exp.tex <==
% %Please add the following packages if necessary:
% %\usepackage{booktabs, multirow} % for borders and merged ranges
% %\usepackage{soul}% for underlines
% %\usepackage[table]{xcolor} % for cell colors
% %\usepackage{changepage,threeparttable} % for wide tables
% %If the table is too wide, replace \begin{table}[!htp]...\end{table} with
% %\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
% \begin{table*}[!htp]\centering
% \scriptsize
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{lrrrrrrrrrrrrrrrrrr}\toprule
% \multirow{2}{*}{\textbf{Data source}} &\multirow{2}{*}{\textbf{Settings}} &\multicolumn{3}{c}{\textbf{Exact Match}} & &\multicolumn{3}{c}{\textbf{No Alif / Ya Errors}} & &\multicolumn{3}{c}{\textbf{No Punctuation}} & &\multicolumn{3}{c}{\textbf{No Puncation and Alif / Ya Errors}} & \\\cmidrule{3-5}\cmidrule{7-9}\cmidrule{11-13}\cmidrule{15-17}
% & &\textbf{Precision} &\textbf{Recall} &\textbf{F\_1.0 } &\textbf{F\_0.5} &\textbf{Precision} &\textbf{Recall} &\textbf{F\_1.0 } &\textbf{F\_0.5} &\textbf{Precision} &\textbf{Recall} &\textbf{F\_1.0 } &\textbf{F\_0.5} &\textbf{Precision} &\textbf{Recall} &\textbf{F\_1.0 } &\textbf{F\_0.5} \\\midrule
% \multirow{5}{*}{Rule-Based} &100k &73.63 &64.28 &68.64 &71.55 &62.83 &52.89 &57.43 &60.55 &87.39 &83.79 &85.56 &86.65 &81.06 &68.98 &74.54 &78.32 \\
% &200k &73.72 &63.60 &68.29 &71.45 &62.76 &51.95 &56.85 &60.25 &87.24 &83.53 &85.34 &86.47 &80.56 &68.60 &74.10 &77.85 \\
% &300k &73.49 &63.42 &68.09 &71.23 &62.36 &51.62 &56.49 &59.87 &87.34 &83.67 &85.46 &86.58 &80.68 &68.74 &74.24 &77.97 \\
% &400k &73.25 &63.99 &68.31 &71.19 &62.24 &52.46 &56.30 &60.00 &87.19 &83.94 &85.53 &86.52 &80.47 &69.30 &74.47 &77.96 \\
% &500k &73.63 &63.86 &68.40 &71.44 &62.73 &52.32 &57.06 &60.33 &87.27 &83.91 &85.55 &86.58 &80.54 &69.36 &74.54 &78.02 \\\
% &1m &73.20 &64.98 & 68.85 & & 62.51 & 54.09 & 57.99 & & 87.17 & 83.86 & 85.48 & & 80.43 & 69.28 & 74.44 & & \\ \midrule
% \multirow{6}{*}{Corruptor} &100k &73.39 &64.12 &68.44 &71.33 &62.57 &52.80 &57.27 &60.34 &86.90 &83.23 &85.03 &86.14 &79.97 &68.24 &73.64 &77.31 \\
% &200k &73.55 &64.28 &68.60 &71.49 &62.74 &53.01 &57.47 &60.52 &86.88 &83.41 &85.11 &86.16 &79.88 &68.50 &73.76 &77.31 \\
% &300k &73.73 &63.90 &68.46 &71.53 &62.83 &52.37 &57.12 &60.42 &86.84 &83.45 &85.11 &86.14 &79.81 &68.46 &73.70 &77.25 \\
% &400k &73.68 &64.24 &68.63 &71.58 &62.88 &52.95 &57.49 &60.61 &86.90 &83.45 &85.14 &86.19 &79.92 &68.76 &73.92 &77.41 \\
% &500k &73.91 &64.45 &68.86 &71.80 &63.22 &53.14 &57.74 &60.91 &87.00 &83.60 &85.26 &86.30 &80.05 &68.82 &74.01 &77.52 \\
% &1m &73.87 &64.53 &68.88 &71.79 &63.17 &53.27 &57.79 &60.91 &86.94 &83.93 &85.41 &86.32 &80.02 &69.52 &74.40 &77.67 \\\midrule
% \multirow{5}{*}{Multi Task Settings} &morph &73.30 &65.00 &\textbf{68.90} &71.47 &62.63 &53.95 &57.97 &60.68 &87.02 &84.12 &85.54 &86.42 &80.37 &69.76 &74.69 &78.00 \\
% &tokenize &73.22 &64.92 &68.82 &71.39 &62.53 &53.96 &57.93 &60.60 &87.01 &84.52 &85.75 &86.50 &80.30 &70.48 &75.07 &78.12 \\
% &detect &73.20 &64.50 &68.57 &71.28 &62.45 &53.35 &57.54 &60.39 &86.94 &84.05 &85.47 &86.35 &80.23 &69.60 &74.54 &77.85 \\
% &error &73.38 &64.45 &68.62 &71.40 &62.58 &53.14 &57.47 &60.43 &86.99 &84.28 &85.61 &86.43 &80.22 &69.82 &74.66 &77.90 \\
% %&multi-task &73.56 &64.05 &68.48 &71.44 &62.75 &52.68 &57.27 &60.44 &86.90 &83.06 &84.93 &86.10 &80.01 &67.88 &73.45 &77.25 \\
% &multi-task combined & 72.77 &  66.14 & 69.30 & & 62.37 & 55.67&  58.83 & & 86.62 & 84.44& 85.51 & & 79.67 & 70.34 & 74.71 \\
% \bottomrule
% \end{tabular}}
% \caption{Performance comparison of different Language Learning Models and configurations on Arabic grammar correction tasks. The table presents metrics including precision, recall, and F-measures for Exact Match, No Alif/Ya Errors, No Punctuation, and No Punctuation and Alif/Ya Errors settings. The results are demonstrated across different data sources and settings to highlight the varying proficiency of these models.}\label{table: seq2seq}
% \end{table*}

%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\scriptsize
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lrrrrr}\toprule
\multirow{2}{*}{\textbf{Settings}} &\multicolumn{4}{c}{\textbf{Exact Match}} \\\cmidrule{2-5}
&\textbf{Precision} &\textbf{Recall} &\textbf{F\_1.0 } &\textbf{F\_0.5} \\\midrule
\textbf{Multi Task Settings} & & & & \\
+morph &73.30 &65.00 &68.90 &71.47  \\
+tokenize &73.22 &64.92 &68.82 &71.39  \\
+detect &73.20 &64.50 &68.57 &71.28 \\
+error &73.38 &64.45 &68.62 &71.40 \\
+combined &72.77 &66.14 &\textbf{69.30} &71.34\\
\bottomrule
\end{tabular}}
\caption{In this table we present the multi-task settings that we used for Training AraT5x}\label{tab: multitask}
\end{table}

==> Tables/seq_corrupt.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\scriptsize
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lrrrrrr}\toprule
\multirow{2}{*}{\textbf{Data source}} &\multirow{2}{*}{\textbf{Settings}} &\multicolumn{3}{c}{\textbf{Exact Match}} & \\\cmidrule{3-5}
& &\textbf{Precision} &\textbf{Recall} &\textbf{F\textsubscript{1.0} } &\textbf{F\textsubscript{0.5}} \\\midrule
\multirow{6}{*}{\textbf{Rule-Based}} $&$100$K&$73.63 $&$64.28 $&$68.64 &$71.55$ \\
&$200$K&$73.72 $&$63.60 $&$68.29 $&$71.45$ \\
&$300$K&$73.49 $&$63.42 $&$68.09 $&$71.23$ \\
&$400$K&$73.25 $&$63.99 $&$68.31 $&$71.19$ \\
&$500$K&$73.63 $&$63.86 $&$68.40 $&$71.44$ \\
&$1$M&$73.20 $&$64.98 $&$68.85 $&$71.39$ \\\midrule
\multirow{6}{*}{\textbf{Corruptor}} $&$100$K&$73.39 $&$64.12 $&$68.44 &$71.33$\\
&$200$K&$73.55 $&$64.28 $&$68.60 $&$71.49$\\
&$300$K&$73.73 $&$63.90 $&$68.46 $&$71.53$\\
&$400$K&$73.68 $&$64.24 $&$68.63 $&$71.58$\\
&$500$K&$73.91 $&$64.45 $&$68.86 $&$71.80$\\
&$1 $M&$73.87 $&$64.53 $&$68.88 $&$71.79$ \\
\bottomrule
\end{tabular}}
\caption{Performance comparison of different Language Learning Models and configurations on Arabic grammar correction tasks. }\label{tab:seq2seq_corrput}
\end{table}


==> Tables/subfigure_chatgpt.tex <==
% \begin{figure*}[t!]
%     \centering
%        \begin{subfigure}\textwidth}
%         \centering
%         \includegraphics[height=1.2in]{Images/Chatgpt_data.png}
%         \label{fig:chatGPT_data}
%     \end{subfigure}%
  
%     ~ 
%     \begin{subfigure}\textwidth}
%         \centering
%         \includegraphics[height=1.2in]{Images/Chatgpt_qalb.png}
%         \label{fig:chatGPT_qalb}
%     \end{subfigure}% 
%     ~ 
%   \begin{subfigure}\textwidth}
%         \centering
%         \includegraphics[height=1.2in]{Images/Chatgpt_random.png}
%         \label{fig:chatGPT_random}
%     \end{subfigure}%
%     \caption{Results for all experiment using ChatGPT}
%     \label{fig:subfigure_chatgpt}
% \end{\figure*}






==> Tables/sufigure_data.tex <==
% \begin{figure*}[t!]
%     \centering
%     \begin{subfigure}{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.2in]{Images/2014_line.png}
%         % \caption
%         \label{fig:2014line}
%     \end{subfigure}%

%     \begin{subfigure}{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.2in]{Images/2015_line.png}
%         % \caption
%         \label{fig:2015_line}
%     \end{subfigure}
%     \caption{Results for all experiment using ChatGPT for data augmentation}
%     \label{fig:subfiguredata}
% \end{figure*}




\begin{figure*}[htbp]
     \centering
     \begin{subfigure}[b]{width=0.1\textwidth}
         \centering
         \includegraphics[scale=0.01]{Images/2014_line.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.1\textwidth}
         \centering
      \includegraphics[scale=0.01]{Images/2015_line.png}
     \end{subfigure}
     %      \hfill
     %  \begin{subfigure}[b]{0.4\textwidth}
     %     \centering
     %     \includegraphics[width=\textwidth]{figs/samples/demo3.png}
     % \end{subfigure}
     %      \hfill
     %  \begin{subfigure}[b]{0.4\textwidth}
     %     \centering
     %     \includegraphics[width=\textwidth]{figs/samples/demo4.png}
     % \end{subfigure}
     \hfill
     
        \caption{Results for all experiment using ChatGPT}
        \label{fig:three graphs}
\end{figure*}






% \begin{figure*}[h]
% \begin{subfigure}[b]{0.49\textwidth}
%   \includegraphics[width=\textwidth]{Images/2015_line.png}
%   % \caption{Results for all experiment using ChatGPT for data augmentation}
% \end{subfigure}
% \begin{subfigure}[b]{0.50\textwidth}
%   \includegraphics[width=\textwidth]{Images/2015_line.png}
%   % \caption{Plot of engine efficiency and break power at the constant speed of 1500 RPM}
% \end{subfigure}
%  \caption{Results for all experiment using ChatGPT for data augmentation}
% \end{figure*} \label{fig:2014line}


==> Tables/test_image.tex <==
\begin{figure*}
     \centering
% First row with two images
\begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Images/zeroshot.png}
    \caption{Model trained only on ChatGPT dataset}
    \label{fig:y equals x}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Images/qalb_finetuned.png}
    \caption{Model further fine-tuned on selected QALB dataset}
    \label{fig:three sin x}
\end{subfigure}

% New line
\vspace{1cm} % Adjust this space according to your needs

% Second row with one image
\begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Images/random_finetuned.png}
    \caption{Model further fine-tuned on selected corruptor dataset}
    \label{fig:five over x}
\end{subfigure}

\caption{F\textsubscript{1} scores for systems trained on 100k to 1m sentences of parallel data}
\label{fig:three graphs}

\end{figure*}


==> Tables/top4_2014_2015_exactmatch.tex <==
\begin{table*}[!htp]\centering
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{llrrrrrrrr}\toprule
\multirow{2}{*}{\textbf{Settings}} &\multirow{2}{*}{\textbf{Models}} &\multicolumn{4}{c}{\textbf{QALB-2014}} &\multicolumn{3}{c}{\textbf{QALB-2015}} \\\cmidrule{3-10}
& &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} \\\midrule
\multirow{5}{*}{\textbf{Encoder-Only }} &AraT5 (11m) &65.60 &44.20 &52.81 &59.81 &72.38 &48.75 &58.26 &65.98 \\
&ARBERTv2 3 Stage &65.00 &41.20 &50.43 &58.27 &75.50 &44.50 &56.00 &66.27 \\
&GPT4 5-shot &64.60 &43.20 &51.78 &58.78 &73.72 &44.16 &55.23 &65.02 \\

\cmidrule{2-10}
&\hl{\textbf{Nizar}} &65.10 &41.30 &50.54 &58.37 &75.41 &45.52 &56.77 &66.66 \\ \bottomrule
\end{tabular}}
\caption{Top4 performing models under No Alif / Ya Errors and No Punctuation normalization methods}\label{tab: top4_2014_2015}
\end{table*}


==> Tables/top4_2014_elsematch.tex <==
\begin{table*}[!htp]\centering
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrr}\toprule
\multirow{2}{*}{\textbf{Settings}} &\multirow{2}{*}{\textbf{Models}} &\multicolumn{4}{c}{\textbf{No Alif / Ya Errors}} &\multicolumn{4}{c}{\textbf{No Punctuation}} &\multicolumn{4}{c}{\textbf{No Punctuation and Alif / Ya Errors}} \\\cmidrule{3-14}
& &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} &\textbf{P} &\textbf{R} &\textbf{F\textsubscript{1.0}} &\textbf{F\textsubscript{0.5}} \\\midrule
\multirow{4}{*}{\textbf{Encoder-Only }} &AraT5 (11m) &62.04 &52.69 &56.99 &59.91 &86.57 &82.70 &84.59 &85.77 &79.32 &67.19 &72.75 &76.56 \\
&ARBERTv2 3 Stage &65.00 &41.20 &50.43 &58.27 &75.50 &44.50 &56.00 &66.27 &55.70 &27.50 &36.82 &46.22 \\
&GPT4 5-shot &64.60 &43.20 &51.78 &58.78 &73.72 &44.16 &55.23 &65.02 &56.80 &34.20 &42.69 &50.17 \\
&\hl{Nizar} &65.10 &41.30 &50.54 &58.37 &75.41 &45.52 &56.77 &66.66 &56.00 &29.20 &38.38 &47.31 \\\
& SOTA &65.10 &41.30 &50.54 &58.37 &75.41 &45.52 &56.77 &66.66 &56.00 &29.20 &38.38 &47.31 \\\bottomrule
\end{tabular}}
\caption{QALB-2014 performing models under else match}\label{tab: top4_others}
\end{table*}


==> Tables/transformers_2014_new.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrrrr}\toprule
&\multicolumn{6}{c}{\textbf{QALB 2014 (M^2)}} \\\cmidrule{2-7}
&\multicolumn{3}{c}{\textbf{Exact Match}} &\multicolumn{3}{c}{\textbf{No Alif / Ya}} \\\cmidrule{2-7}
&\textbf{Precision} &\textbf{Recall} &\textbf{F\textsubscript{1}} &\textbf{Precision} &\textbf{Recall} &\textbf{F\textsubscript{1}} \\\midrule
\textbf{AraBart} &$\underline{70.03}$ &$\underline{61.00}$ &$\underline{65.2}$ &$\underline{58.46}$ &$\underline{49.47}$ &$\underline{53.59}$ \\
\textbf{AraT5} &$\textbf{72.46}$ &$\textbf{64.23}$ &$\textbf{68.1}$ &$\textbf{61.58}$ &$\textbf{53.07}$ &$\textbf{57.01}$ \\
\textbf{mT0} &$68.81$ &$52.99$ &$59.87$ &$55.64$ &$39.56$ &$46.25$ \\
\textbf{mT5} &$68.53$ &$52.78$ &$59.64$ &$55.34$ &$39.43$ &$46.05$ 
\\\midrule
&\multicolumn{3}{c}{\textbf{No Punct}} &\multicolumn{3}{c}{\textbf{No Alif /Ya and Punct}} \\\cmidrule{2-7}
&\textbf{Precision} &\textbf{Recall} &\textbf{F\textsubscript{1}} &\textbf{Precision} &\textbf{Recall} &\textbf{F\textsubscript{1}} \\\midrule
\textbf{AraBart} &$83.01$ &$76.82$ &$79.8$ &$72.09$ &$58.46$ &$64.56$ \\
\textbf{AraT5} &$\textbf{86.28}$ &$\textbf{82.30}$ &$\textbf{84.25}$ &$\textbf{78.99}$ &$\textbf{66.67}$ &$\textbf{72.31}$ \\
\textbf{mT0} &$79.51$ &$69.22$ &$74.01$ &$65.97$ &$47.61$ &$55.31$ \\
\textbf{mT5} &$79.15$ &$68.44$ &$73.41$ &$64.83$ &$46.49$ &$54.10$ \\
\bottomrule
\end{tabular}}
\caption{Performance of transformer-based models on the QALB 2014 dataset. Bold values indicate the highest scores in Precision, Recall, and F\textsubscript{1}.}\label{tab:tf_2014}
\end{table}

==> Tables/transformers_error_type_2014.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{tabular}{lllll}
                                &                                 & F1 Score            &                     &                     \\
\cellcolor[HTML]{FFFFFF}Err Tag & \cellcolor[HTML]{FFFFFF}AraBart & AraT5               & mT0                 & mT5                 \\
OH                              & 0.9471919530595140              & 0.958303005095144   & 0.9228326452842170  & 0.9209745762711870  \\
OT                              & 0.9315673289183220              & 0.9601737871107890  & 0.8995502248875560  & 0.8897280966767370  \\
OA                              & 0.8320312500000000              & 0.8914285714285720  & 0.8016359918200410  & 0.7842323651452280  \\
OW                              & 0.8666666666666670              & 0.8942307692307690  & 0.7853403141361260  & 0.7643979057591620  \\
ON                              & 0.0                             & 0.0                 & 0.0                 & 0.0                 \\
OG                              & 0.5185185185185190              & 0.6101694915254240  & 0.5283018867924530  & 0.45833333333333300 \\
OC                              & 0.3225806451612900              & 0.5581395348837210  & 0.28571428571428600 & 0.3333333333333330  \\
OR                              & 0.5439624853458380              & 0.728421052631579   & 0.37984496124031000 & 0.3682864450127880  \\
OD                              & 0.5668604651162790              & 0.6715116279069770  & 0.4056603773584910  & 0.40249609984399400 \\
OM                              & 0.585438335809807               & 0.6834030683403070  & 0.397887323943662   & 0.38566552901023900 \\
OO                              & 0.0                             & 0.0                 & 0.0                 & 0.0                 \\
MI                              & 0.16326530612244900             & 0.291970802919708   & 0.10344827586206900 & 0.06896551724137930 \\
MT                              & 0.0                             & 0.3333333333333330  & 0.0                 & 0.0                 \\
XC                              & 0.5005988023952100              & 0.5538461538461540  & 0.23765432098765400 & 0.20754716981132100 \\
XF                              & 0.22222222222222200             & 0.31111111111111100 & 0.0                 & 0.0                 \\
XG                              & 0.3548387096774190              & 0.3090909090909090  & 0.23636363636363600 & 0.1568627450980390  \\
XN                              & 0.30864197530864200             & 0.43636363636363600 & 0.14388489208633100 & 0.11851851851851900 \\
XT           & 0.04448398576512460 & 0.047619047619047600 & 0.024987986544930300 & 0.023126734505087900 \\
XM                              & 0.03669724770642200             & 0.12962962962963000 & 0.01851851851851850 & 0.01941747572815530 \\
XO                              & 0.0                             & 0.0                 & 0.0                 & 0.0                 \\
SW                              & 0.42190669371196800             & 0.5233644859813080  & 0.34697855750487300 & 0.33398821218074700 \\
SF                              & 0.0                             & 0.0                 & 0.0                 & 0.0                 \\
PC                              & 0.48026868178001700             & 0.514480408858603   & 0.48591549295774600 & 0.4995633187772930  \\
PT                              & 0.2541613316261200              & 0.24267782426778200 & 0.2472981563890660  & 0.25071405902888000 \\
PM                              & 0.4593012945557720              & 0.48014215904042600 & 0.3849662832209440  & 0.3939754260800640  \\
MG                              & 0.7888040712468190              & 0.8205128205128210  & 0.7311258278145700  & 0.7217043941411450  \\
SP                              & 0.9039623908663530              & 0.9484536082474230  & 0.8861952861952860  & 0.8694463431305540  \\
                                &                                 &                     &                     &                     \\
micro avg    & 0.6173661111270480  & 0.6484015655800930   & 0.5547096317280450   & 0.552409017238839    \\
macro avg    & 0.40940630968817700 & 0.47771766070278400  & 0.3427446387267690   & 0.3322695406898960   \\
weighted avg & 0.6615944013346200  & 0.6941651935462590   & 0.5994830225169000   & 0.5981057693508090  
\end{tabular}
\end{table}

==> Tables/transformers_error_type_2015.tex <==
\begin{table}[]
\begin{tabular}{lllllllllllll}
                &  &           & \textbf{}   &    &  &           & \textbf{QALB2015} & \textbf{} &  &      &                     &    \\
\textbf{}       &  & \textbf{} & \textbf{No Alif / Ya Error} &    &  & \textbf{} & \textbf{No Punctuation}    & \textbf{} &  &      & \textbf{Bert-Score} &    \\ \hline
\textbf{No Alif / Ya and Punctuation} &  & Pre       & Rec.        & F1 &  & Pre.      & Rec.              & F1        &  & Pre. & Rec.                & F1 \\ \hline
AraBART &  & 0.5 &  &  &  &  &  &  &  &  &  &  \\
AraT5   &  &     &  &  &  &  &  &  &  &  &  &  \\
mT0     &  &     &  &  &  &  &  &  &  &  &  &  \\
mT5     &  &     &  &  &  &  &  &  &  &  &  &  \\ \hline
        &  &     &  &  &  &  &  &  &  &  &  &  \\
        &  &     &  &  &  &  &  &  &  &  &  & 
\end{tabular}
\end{table}

==> Tables/transformers_result_2015.tex <==
\begin{table}[t]
\centering
 \resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{lrrrrrrr}\toprule
&\multicolumn{6}{c}{\textbf{QALB 2015 (M^2)}} \\\cmidrule{2-7}
&\multicolumn{3}{c}{\textbf{Exact Match}} &\multicolumn{3}{c}{\textbf{No Alif / Ya}} \\\cmidrule{2-7}
&\textbf{Precision} &\textbf{Recall} &\textbf{F\textsubscript{1}} &\textbf{Precision} &\textbf{Recall} &\textbf{F\textsubscript{1}} \\\midrule
\textbf{AraBart} &67.95 &65.62 &66.76 &52.48 &51.84 &52.16 \\
\textbf{AraT5} &\textbf{71.31} &\textbf{73.48} &\textbf{72.38} &\textbf{55.03} &\textbf{56.19} &\textbf{55.61} \\
\textbf{mT0} &67.61 &58.41 &62.67 &50.52 &42.18 &45.97 \\
\textbf{mT5} &67.43 &57.3 &61.95 &50.15 &40.81 &45 \\\hline
&\multicolumn{3}{c}{\textbf{No Punct}} &\multicolumn{3}{c}{\textbf{No Alif /Ya and Punct}} \\\cmidrule{2-7}
&\textbf{Precision} &\textbf{Recall} &\textbf{F\textsubscript{1}} &\textbf{Precision} &\textbf{Recall} &\textbf{F\textsubscript{1}} \\\cmidrule{2-7}
\textbf{AraBart} &84.11 &79.02 &81.49 &73.23 &59.94 &65.92 \\
\textbf{AraT5} &\textbf{86.93} &\textbf{84.57} &\textbf{85.73} &\textbf{74.11} &\textbf{67.02} &\textbf{70.39} \\
\textbf{mT0} &81.41 &71.47 &76.12 &68.27 &48.54 &56.74 \\
\textbf{mT5} &81.18 &70.71 &75.58 &68.04 &47.79 &56.1 \\
\bottomrule
\end{tabular}}
\caption{Performance of transformer-based models on the QALB 2014 and 2015 datasets. Bold values indicate the highest scores in Precision, Recall, and F\textsubscript{1}.}
\end{table}

==> Tables/transformers_results_2014.tex <==
\begin{table}[t]
% \centering
 \resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{clrrrrrr}
\toprule
\multicolumn{1}{l}{}              &                   & \multicolumn{6}{c}{\textbf{QALB 2014 (M^2)}}                                                                                                                                                                                   \\\toprule       
\multicolumn{1}{l}{}              &                   & \multicolumn{3}{c}{\textbf{Exact Match}}                                                                                & \multicolumn{3}{c}{\textbf{No Alif / Ya}}                                                                      \\ 
\cline{3-8}
\multicolumn{1}{l}{}              &                   & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F\textsubscript{1}}} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F\textsubscript{1}}} \\ \cline{3-8}
\multirow{4}{*}{\textbf{ChatGPT}} & \textbf{AraBart}   &
\multicolumn{1}{l}{}                   & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{}            & \multicolumn{1}{l}{}                   & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{}            \\
                                  & \textbf{AraT5}   & $70.03$                                  & $61.00$                               & $65.20$                           & $58.46$                                  & $49.47$                               & $53.59$                           \\
                                  & \textbf{mT0}   & $64.60$                                   & $60.37$                               & $\textbf{62.41}$                  & $\textbf{54.06}$                         & $\textbf{52.51}$                      & $\textbf{53.28}$                  \\
                                  & $\textbf{mT5}$   & $\textbf{64.70}$                          & $59.59$                               & $62.04$                           & $54.01$                                  & $51.28$                               & $52.61$                           \\
                    \\

\toprule
\multicolumn{1}{l}{}              &                   & \multicolumn{3}{c}{\textbf{No Punct}}                                                                                   & \multicolumn{3}{c}{\textbf{No Alif /Ya and Punct}}                                                             \\ \cline{3-8}
\multicolumn{1}{l}{}              &                   & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F\textsubscript{1}}} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F\textsubscript{1}}} \\ \cline{3-8}
\multirow{4}{*}{\textbf{ChatGPT}} & \textbf{AraBart}   & \multicolumn{1}{l}{}                   & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{}            & \multicolumn{1}{l}{}                   & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{}            \\
                                  & \textbf{AraT5}   & $59.81$                                  & $64.35$                               & $62.00$                              & $41.55$                                  & $53.8$                                & $46.89$                           \\
                                  & \textbf{mT0}   & $66.09$                                  & $\textbf{70.88}$                      & $68.40$                            & $48.14$                                  & $\textbf{58.78}$                               & $52.93$                           \\
                                  & \textbf{mT5}   & $66.33$                                  & $70.80$                                & $\textbf{68.49}$                  & $48.63$                                  & $58.48$                               & $\textbf{53.1}$          \\
\toprule
\end{tabular}}
\caption{Performance of transformer-based models on the QALB 2014 dataset. Bold values indicate the highest scores in Precision, Recall, and F\textsubscript{1}.}
\end{table}

==> Tables/zero-shot.tex <==
  \begin{table}[ht]
% \linespread{1.15}
\small
\centering
\resizebox{0.46\textwidth}{!}{
\begin{tabular}{p{1.9cm} | p{6cm}}
\toprule
 \multicolumn{1}{c|}{\textbf{Method}} &  \multicolumn{1}{c}{\textbf{GEC Prompt}} \\
\cmidrule(lr){1-2}
\multirow{10}{*}{\textbf{Zero-shot}} &"role": "system", "content": 'You are an Arabic grammatical error correction tool that can identify and correct grammatical errors in a text. These sentences cover a range of common grammar error types in Arabic, such as word order, verb conjugation, agreement, pronouns, hamza, diacritics, particles, compound words, and case endings.' \\&
 \texttt{"role": "user", "content": 'Please identify and correct any grammatical errors in the following sentence while keeping the original sentence structure unchanged as much as possible: '}\\ 
\cmidrule(lr){1-2}
\multirow{21}{*}{\textbf{Zero-shot CoT}} &"role": "system", "content": 'You are an Arabic grammatical error correction tool that can identify and correct grammatical errors in a text. These sentences cover a range of common grammar error types in Arabic, such as word order, verb conjugation, agreement, pronouns, hamza, diacritics, particles, compound words, and case endings.' \\&
\texttt{"role": "user", "content": 'Please identify and correct any grammatical errors in the following sentence indicated by <input> ERROR </input> tag, you need to comprehend the sentence as a whole before identifying and correcting any errors step by step while keeping the original sentence structure unchanged as much as possible. Afterward, output the corrected version directly without any explanations. Remember to format your corrected output results with the tag <output> Your Corrected Version </output>. Please start: <input> ERROR </input>: ' }\\
\bottomrule
\end{tabular}}
\linespread{1}
\caption{Zero-shot and zero-shot CoT settings for ChatGPT.}
\label{Tab:GEC_zero_shot_prompts}
%\vskip -1em
\end{table}
